SpeechAgents: Human-Communication Simulation with Multi-Modal Multi-Agent Systems

Human communication is a complex and diverse process that not only involves multiple factors such as language, commonsense, and cultural backgrounds but also requires the participation of multimodal information, such as speech. Large Language Model (LLM)-based multi-agent systems have demonstrated promising performance in simulating human society. Can we leverage LLM-based multi-agent systems to simulate human communication? However, current LLM-based multi-agent systems mainly rely on text as the primary medium. In this paper, we propose SpeechAgents, a multi-modal LLM based multi-agent system designed for simulating human communication. SpeechAgents utilizes multi-modal LLM as the control center for individual agent and employes multi-modal signals as the medium for exchanged messages among agents. Additionally, we propose Multi-Agent Tuning to enhance the multi-agent capabilities of LLM without compromising general abilities. To strengthen and evaluate the effectiveness of human communication simulation, we build the Human-Communication Simulation Benchmark. Experimental results demonstrate that SpeechAgents can simulate human communication dialogues with consistent content, authentic rhythm, and rich emotions and demonstrate excellent scalability even with up to 25 agents, which can apply to tasks such as drama creation and audio novels generation. Code and models will be open-sourced at https://github. com/0nutation/SpeechAgents

==> Sections/010_intro_v0.tex <==
The rise of large language models~(LLM)-based agents has garnered significant attention~\cite{openai2023gpt4, Significant_Gravitas_AutoGPT, li2023camel}, as they prove helpful in assisting humans with various complex tasks. These agents not only facilitate individual tasks but also engage in communication and collaboration with other agents~\cite{talebirad2023multiagent, chen2023agentverse}, contributing to the construction of multi-agent systems. This collaborative effort aims to enhance task accuracy~\cite{qian2023communicative, hong2023metagpt} and simulate real-world scenarios effectively~\cite{park2023generative}.
Human communication, a nuanced and complex process, involves a myriad of factors such as language, emotions, non-verbal expressions, and cultural backgrounds~\cite{devito2018human}. Leveraging LLM-based agents for simulating human communication aids in exploring the mechanisms underlying human cognition and social interactions, shedding light on the intricacies of these fundamental aspects~\cite{troitzsch2012simulating}.

In human communication, apart from linguistic elements, multi-modal information is commonly employed, encompassing modalities such as speech, gestures, and facial expressions~\cite{holler2019multimodal}. However, current LLM-based multi-agent systems predominantly rely on text as the primary medium for information exchange~\cite{talebirad2023multiagent, chen2023agentverse}, often lacking effective processing and utilization of other non-textual modalities such as speech. To achieve a more authentic simulation of Human-Communication, the incorporation of multi-modal signals becomes necessary.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{Figures/mas.png} 
\caption{LLM-based Multi-Agent System is built on text-based LLM and rely on text as the medium for information exchange. Multi-modal LLM-based Multi-Agent System is built on multi-modal LLM and rely on multi-modal signals as the medium for information exchange}
\label{fig:mas}
\end{figure}

Current multi-modal agents primarily utilize text-based LLM as the central control hub, interacting with other modalities through tool use of modality-specific experts~\cite{shen2023hugginggpt,yang2023mmreact,wu2023visual,huang2023audiogpt}. In such system, multi-modal capabilities are not inherently ingrained in agents, unlike text, posing challenges for seamless information integration and knowledge transfer across modalities. Furthermore, current exploration of multi-modal agents focus on individual agents~\cite{li2023multimodal}, lacking exploration into the construction of a multi-modal LLM-based multi-agent system for accomplishing complex tasks or simulating real-world scenarios.
Hence, there is a need to develop a multi-modal LLM-based multi-agent system, where multiple multi-modal agents collaborate to simulate authentic human communication through speech dialogues and the exchange of multi-modal information. 

We propose SpeechAgents, a multi-modal LLM based multi-agent system designed to simulate human communication. We adopt SpeechGPT~\cite{zhang-etal-2023-speechgpt}, a cross-modal LLM that supports multi-modal input and output, as the centrol centor for agents. SpeechGPT possesses intrinsic cross-modal capabilities, allowing for direct spoken dialogues.
To assess and enhance the multi-modal human communication simulation capabilities, we introduce the Human-Communication Simulation Benchmark. We build multi-modal multi-agent system and propose multi-agent tuning to improve the multi-agent capabilities of the LLM. Experimental results demonstrate that SpeechAgents can generate human-like communication dialogues with accurate content, authentic rhythm, and rich emotions. It successfully accomplishes tasks such as drama creation and audio novels generation.









==> rebib_custom.tex <==
@inproceedings{lee2022textless,
 address = {Seattle, United States},
 author = {Lee, Ann  and
Gong, Hongyu  and
Duquenne, Paul-Ambroise  and
Schwenk, Holger  and
Chen, Peng-Jen  and
Wang, Changhan  and
Popuri, Sravya  and
Adi, Yossi  and
Pino, Juan  and
Gu, Jiatao  and
Hsu, Wei-Ning},
 booktitle = {Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
 doi = {10.18653/v1/2022.naacl-main.63},
 pages = {860--872},
 publisher = {Association for Computational Linguistics},
 title = {Textless Speech-to-Speech Translation on Real Data},
 url = {https://aclanthology.org/2022.naacl-main.63},
 year = {2022}
}

@article{lakhotia2021generative,
 address = {Cambridge, MA},
 author = {Lakhotia, Kushal  and
Kharitonov, Eugene  and
Hsu, Wei-Ning  and
Adi, Yossi  and
Polyak, Adam  and
Bolte, Benjamin  and
Nguyen, Tu-Anh  and
Copet, Jade  and
Baevski, Alexei  and
Mohamed, Abdelrahman  and
Dupoux, Emmanuel},
 doi = {10.1162/tacl_a_00430},
 journal = {Transactions of the Association for Computational Linguistics},
 pages = {1336--1354},
 publisher = {MIT Press},
 title = {On Generative Spoken Language Modeling from Raw Audio},
 url = {https://aclanthology.org/2021.tacl-1.79},
 volume = {9},
 year = {2021}
}

@article{inaguma2022unity,
 author = {Inaguma, Hirofumi and Popuri, Sravya and Kulikov, Ilia and Chen, Peng-Jen and Wang, Changhan and Chung, Yu-An and Tang, Yun and Lee, Ann and Watanabe, Shinji and Pino, Juan},
 journal = {ArXiv preprint},
 title = {UnitY: Two-pass Direct Speech-to-speech Translation with Discrete Units},
 url = {https://arxiv.org/abs/2212.08055},
 volume = {abs/2212.08055},
 year = {2022}
}

@article{popuri2022enhanced,
 author = {Popuri, Sravya and Chen, Peng-Jen and Wang, Changhan and Pino, Juan and Adi, Yossi and Gu, Jiatao and Hsu, Wei-Ning and Lee, Ann},
 journal = {ArXiv preprint},
 title = {Enhanced Direct Speech-to-Speech Translation Using Self-supervised Pre-training and Data Augmentation},
 url = {https://arxiv.org/abs/2204.02967},
 volume = {abs/2204.02967},
 year = {2022}
}

@article{huang2022transpeech,
 author = {Huang, Rongjie and Zhao, Zhou and Liu, Jinglin and Liu, Huadai and Ren, Yi and Zhang, Lichao and He, Jinzheng},
 journal = {ArXiv preprint},
 title = {TranSpeech: Speech-to-Speech Translation With Bilateral Perturbation},
 url = {https://arxiv.org/abs/2205.12523},
 volume = {abs/2205.12523},
 year = {2022}
}

@inproceedings{kharitonov2022text,
 address = {Dublin, Ireland},
 author = {Kharitonov, Eugene  and
Lee, Ann  and
Polyak, Adam  and
Adi, Yossi  and
Copet, Jade  and
Lakhotia, Kushal  and
Nguyen, Tu Anh  and
Riviere, Morgane  and
Mohamed, Abdelrahman  and
Dupoux, Emmanuel  and
Hsu, Wei-Ning},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.593},
 pages = {8666--8681},
 publisher = {Association for Computational Linguistics},
 title = {Text-Free Prosody-Aware Generative Spoken Language Modeling},
 url = {https://aclanthology.org/2022.acl-long.593},
 year = {2022}
}

@article{chen2022wavlm,
 author = {Chen, Sanyuan and Wang, Chengyi and Chen, Zhengyang and Wu, Yu and Liu, Shujie and Chen, Zhuo and Li, Jinyu and Kanda, Naoyuki and Yoshioka, Takuya and Xiao, Xiong and others},
 journal = {IEEE Journal of Selected Topics in Signal Processing},
 number = {6},
 pages = {1505--1518},
 publisher = {IEEE},
 title = {Wavlm: Large-scale self-supervised pre-training for full stack speech processing},
 volume = {16},
 year = {2022}
}

@inproceedings{chung2021w2v,
 author = {Chung, Yu-An and Zhang, Yu and Han, Wei and Chiu, Chung-Cheng and Qin, James and Pang, Ruoming and Wu, Yonghui},
 booktitle = {2021 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
 organization = {IEEE},
 pages = {244--250},
 title = {W2v-bert: Combining contrastive learning and masked language modeling for self-supervised speech pre-training},
 year = {2021}
}

@article{zhang2022speechlm,
 author = {Zhang, Ziqiang and Chen, Sanyuan and Zhou, Long and Wu, Yu and Ren, Shuo and Liu, Shujie and Yao, Zhuoyuan and Gong, Xun and Dai, Lirong and Li, Jinyu and others},
 journal = {ArXiv preprint},
 title = {Speechlm: Enhanced speech pre-training with unpaired textual data},
 url = {https://arxiv.org/abs/2209.15329},
 volume = {abs/2209.15329},
 year = {2022}
}

@inproceedings{berard2016listen,
 author = {B{\'e}rard, Alexandre and Pietquin, Olivier and Besacier, Laurent and Servan, Christophe},
 booktitle = {NIPS Workshop on end-to-end learning for speech and audio processing},
 title = {Listen and Translate: A Proof of Concept for End-to-End Speech-to-Text Translation},
 year = {2016}
}

@inproceedings{di2019adapting,
 author = {Mattia Antonino Di Gangi and
Matteo Negri and
Marco Turchi},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/GangiNT19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-3045},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {1133--1137},
 publisher = {{ISCA}},
 timestamp = {Fri, 29 Jan 2021 00:00:00 +0100},
 title = {Adapting Transformer to End-to-End Spoken Language Translation},
 url = {https://doi.org/10.21437/Interspeech.2019-3045},
 year = {2019}
}

@inproceedings{gaido2021ctc,
 address = {Online},
 author = {Gaido, Marco  and
Cettolo, Mauro  and
Negri, Matteo  and
Turchi, Marco},
 booktitle = {Proceedings of the 16th Conference of the European Chapter of the Association for Computational Linguistics: Main Volume},
 doi = {10.18653/v1/2021.eacl-main.57},
 pages = {690--696},
 publisher = {Association for Computational Linguistics},
 title = {{CTC}-based Compression for Direct Speech Translation},
 url = {https://aclanthology.org/2021.eacl-main.57},
 year = {2021}
}

@inproceedings{dong2021listen,
 author = {Dong, Qianqian and Ye, Rong and Wang, Mingxuan and Zhou, Hao and Xu, Shuang and Xu, Bo and Li, Lei},
 booktitle = {Proc. of AAAI},
 pages = {12749--12759},
 title = {Listen, understand and translate: Triple supervision decouples end-to-end speech-to-text translation},
 year = {2021}
}

@inproceedings{dong2021consecutive,
 author = {Dong, Qianqian and Wang, Mingxuan and Zhou, Hao and Xu, Shuang and Xu, Bo and Li, Lei},
 booktitle = {Proc. of AAAI},
 pages = {12738--12748},
 title = {Consecutive decoding for speech-to-text translation},
 year = {2021}
}

@inproceedings{xu2021stacked,
 address = {Online},
 author = {Xu, Chen  and
Hu, Bojie  and
Li, Yanyang  and
Zhang, Yuhao  and
Huang, Shen  and
Ju, Qi  and
Xiao, Tong  and
Zhu, Jingbo},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.204},
 pages = {2619--2630},
 publisher = {Association for Computational Linguistics},
 title = {Stacked Acoustic-and-Textual Encoding: Integrating the Pre-trained Models into Speech Translation Encoders},
 url = {https://aclanthology.org/2021.acl-long.204},
 year = {2021}
}

@inproceedings{zhang2020adaptive,
 address = {Online},
 author = {Zhang, Biao  and
Titov, Ivan  and
Haddow, Barry  and
Sennrich, Rico},
 booktitle = {Findings of the Association for Computational Linguistics: EMNLP 2020},
 doi = {10.18653/v1/2020.findings-emnlp.230},
 pages = {2533--2544},
 publisher = {Association for Computational Linguistics},
 title = {Adaptive Feature Selection for End-to-End Speech Translation},
 url = {https://aclanthology.org/2020.findings-emnlp.230},
 year = {2020}
}

@inproceedings{wang2021voxpopuli,
 address = {Online},
 author = {Wang, Changhan  and
Riviere, Morgane  and
Lee, Ann  and
Wu, Anne  and
Talnikar, Chaitanya  and
Haziza, Daniel  and
Williamson, Mary  and
Pino, Juan  and
Dupoux, Emmanuel},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.80},
 pages = {993--1003},
 publisher = {Association for Computational Linguistics},
 title = {{V}ox{P}opuli: A Large-Scale Multilingual Speech Corpus for Representation Learning, Semi-Supervised Learning and Interpretation},
 url = {https://aclanthology.org/2021.acl-long.80},
 year = {2021}
}

@inproceedings{di2019must,
 address = {Minneapolis, Minnesota},
 author = {Di Gangi, Mattia A.  and
Cattoni, Roldano  and
Bentivogli, Luisa  and
Negri, Matteo  and
Turchi, Marco},
 booktitle = {Proc. of NAACL-HLT},
 doi = {10.18653/v1/N19-1202},
 pages = {2012--2017},
 publisher = {Association for Computational Linguistics},
 title = {{M}u{ST}-{C}: a {M}ultilingual {S}peech {T}ranslation {C}orpus},
 url = {https://aclanthology.org/N19-1202},
 year = {2019}
}

@inproceedings{wang2021covost,
 author = {Changhan Wang and
Anne Wu and
Jiatao Gu and
Juan Pino},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/WangWGP21.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-2027},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {2247--2251},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {CoVoST 2 and Massively Multilingual Speech Translation},
 url = {https://doi.org/10.21437/Interspeech.2021-2027},
 year = {2021}
}

@inproceedings{zhao2021neurst,
 address = {Online},
 author = {Zhao, Chengqi  and
Wang, Mingxuan  and
Dong, Qianqian  and
Ye, Rong  and
Li, Lei},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-demo.7},
 pages = {55--62},
 publisher = {Association for Computational Linguistics},
 title = {{N}eur{ST}: Neural Speech Translation Toolkit},
 url = {https://aclanthology.org/2021.acl-demo.7},
 year = {2021}
}

@inproceedings{du2022regularizing,
 author = {Du, Yichao and Zhang, Zhirui and Wang, Weizhi and Chen, Boxing and Xie, Jun and Xu, Tong},
 booktitle = {Proc. of AAAI},
 pages = {10590--10598},
 title = {Regularizing end-to-end speech translation with triangular decomposition agreement},
 year = {2022}
}

@inproceedings{pino2020selfa,
 author = {Juan Miguel Pino and
Qiantong Xu and
Xutai Ma and
Mohammad Javad Dousti and
Yun Tang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/PinoXMDT20.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2020-2938},
 editor = {Helen Meng and
Bo Xu and
Thomas Fang Zheng},
 pages = {1476--1480},
 publisher = {{ISCA}},
 timestamp = {Thu, 12 Aug 2021 01:00:00 +0200},
 title = {Self-Training for End-to-End Speech Translation},
 url = {https://doi.org/10.21437/Interspeech.2020-2938},
 year = {2020}
}

@inproceedings{inaguma2020espnet,
 address = {Online},
 author = {Inaguma, Hirofumi  and
Kiyono, Shun  and
Duh, Kevin  and
Karita, Shigeki  and
Yalta, Nelson  and
Hayashi, Tomoki  and
Watanabe, Shinji},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2020.acl-demos.34},
 pages = {302--311},
 publisher = {Association for Computational Linguistics},
 title = {{ESP}net-{ST}: All-in-One Speech Translation Toolkit},
 url = {https://aclanthology.org/2020.acl-demos.34},
 year = {2020}
}

@inproceedings{papi2021speechformer,
 address = {Online and Punta Cana, Dominican Republic},
 author = {Papi, Sara  and
Gaido, Marco  and
Negri, Matteo  and
Turchi, Marco},
 booktitle = {Proc. of EMNLP},
 doi = {10.18653/v1/2021.emnlp-main.127},
 pages = {1698--1706},
 publisher = {Association for Computational Linguistics},
 title = {Speechformer: Reducing Information Loss in Direct Speech Translation},
 url = {https://aclanthology.org/2021.emnlp-main.127},
 year = {2021}
}

@inproceedings{ye2021end,
 author = {Rong Ye and
Mingxuan Wang and
Lei Li},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/YeW021.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-1065},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {2267--2271},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {End-to-End Speech Translation via Cross-Modal Progressive Training},
 url = {https://doi.org/10.21437/Interspeech.2021-1065},
 year = {2021}
}

@inproceedings{ye2022cross,
 address = {Seattle, United States},
 author = {Ye, Rong  and
Wang, Mingxuan  and
Li, Lei},
 booktitle = {Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
 doi = {10.18653/v1/2022.naacl-main.376},
 pages = {5099--5113},
 publisher = {Association for Computational Linguistics},
 title = {Cross-modal Contrastive Learning for Speech Translation},
 url = {https://aclanthology.org/2022.naacl-main.376},
 year = {2022}
}

@inproceedings{tang2021improving,
 address = {Online},
 author = {Tang, Yun  and
Pino, Juan  and
Li, Xian  and
Wang, Changhan  and
Genzel, Dmitriy},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.328},
 pages = {4252--4261},
 publisher = {Association for Computational Linguistics},
 title = {Improving Speech Translation by Understanding and Learning from the Auxiliary Text Translation Task},
 url = {https://aclanthology.org/2021.acl-long.328},
 year = {2021}
}

@inproceedings{zhang2022revisiting,
 author = {Zhang, Biao and Haddow, Barry and Sennrich, Rico},
 booktitle = {Proc. of ICML},
 title = {Revisiting End-to-End Speech-to-Text Translation From Scratch},
 year = {2022}
}

@inproceedings{tang2022unified,
 address = {Dublin, Ireland},
 author = {Tang, Yun  and
Gong, Hongyu  and
Dong, Ning  and
Wang, Changhan  and
Hsu, Wei-Ning  and
Gu, Jiatao  and
Baevski, Alexei  and
Li, Xian  and
Mohamed, Abdelrahman  and
Auli, Michael  and
Pino, Juan},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.105},
 pages = {1488--1499},
 publisher = {Association for Computational Linguistics},
 title = {Unified Speech-Text Pre-training for Speech Translation and Recognition},
 url = {https://aclanthology.org/2022.acl-long.105},
 year = {2022}
}

@inproceedings{fang2022stemm,
 address = {Dublin, Ireland},
 author = {Fang, Qingkai  and
Ye, Rong  and
Li, Lei  and
Feng, Yang  and
Wang, Mingxuan},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.486},
 pages = {7050--7062},
 publisher = {Association for Computational Linguistics},
 title = {{STEMM}: Self-learning with Speech-text Manifold Mixup for Speech Translation},
 url = {https://aclanthology.org/2022.acl-long.486},
 year = {2022}
}

@inproceedings{zheng2021fused,
 author = {Renjie Zheng and
Junkun Chen and
Mingbo Ma and
Liang Huang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/ZhengCM021.bib},
 booktitle = {Proc. of ICML},
 editor = {Marina Meila and
Tong Zhang},
 pages = {12736--12746},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 25 Aug 2021 01:00:00 +0200},
 title = {Fused Acoustic and Text Encoding for Multimodal Bilingual Pretraining
and Speech Translation},
 url = {http://proceedings.mlr.press/v139/zheng21a.html},
 volume = {139},
 year = {2021}
}

@article{karakanta2018neural,
 author = {Karakanta, Alina and Dehdari, Jon and van Genabith, Josef},
 journal = {Machine Translation},
 number = {1},
 pages = {167--189},
 publisher = {Springer},
 title = {Neural machine translation for low-resource languages without parallel corpora},
 volume = {32},
 year = {2018}
}

@inproceedings{anastasopoulos2018tied,
 address = {New Orleans, Louisiana},
 author = {Anastasopoulos, Antonios  and
Chiang, David},
 booktitle = {Proc. of NAACL-HLT},
 doi = {10.18653/v1/N18-1008},
 pages = {82--91},
 publisher = {Association for Computational Linguistics},
 title = {Tied Multitask Learning for Neural Speech Translation},
 url = {https://aclanthology.org/N18-1008},
 year = {2018}
}

@inproceedings{indurthi2021task,
 author = {Indurthi, Sathish and Zaidi, Mohd Abbas and Lakumarapu, Nikhil Kumar and Lee, Beomseok and Han, Hyojung and Ahn, Seokchan and Kim, Sangha and Kim, Chanwoo and Hwang, Inchul},
 booktitle = {Proc. of ICASSP},
 organization = {IEEE},
 pages = {7723--7727},
 title = {Task aware multi-task learning for speech to text tasks},
 year = {2021}
}

@inproceedings{schneider2019wav2vec,
 author = {Steffen Schneider and
Alexei Baevski and
Ronan Collobert and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/SchneiderBCA19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-1873},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {3465--3469},
 publisher = {{ISCA}},
 timestamp = {Fri, 29 Jan 2021 00:00:00 +0100},
 title = {wav2vec: Unsupervised Pre-Training for Speech Recognition},
 url = {https://doi.org/10.21437/Interspeech.2019-1873},
 year = {2019}
}

@inproceedings{dong2018speech,
 author = {Linhao Dong and
Shuang Xu and
Bo Xu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icassp/DongXX18.bib},
 booktitle = {2018 {IEEE} International Conference on Acoustics, Speech and Signal
Processing, {ICASSP} 2018, Calgary, AB, Canada, April 15-20, 2018},
 doi = {10.1109/ICASSP.2018.8462506},
 pages = {5884--5888},
 publisher = {{IEEE}},
 timestamp = {Tue, 25 Jun 2019 01:00:00 +0200},
 title = {Speech-Transformer: {A} No-Recurrence Sequence-to-Sequence Model for
Speech Recognition},
 url = {https://doi.org/10.1109/ICASSP.2018.8462506},
 year = {2018}
}

@inproceedings{baevski2020wav2vec,
 author = {Alexei Baevski and
Yuhao Zhou and
Abdelrahman Mohamed and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/BaevskiZMA20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {wav2vec 2.0: {A} Framework for Self-Supervised Learning of Speech
Representations},
 url = {https://proceedings.neurips.cc/paper/2020/hash/92d1e1eb1cd6f9fba3227870bb6d7f07-Abstract.html},
 year = {2020}
}

@inproceedings{van2017neural,
 author = {A{\"{a}}ron van den Oord and
Oriol Vinyals and
Koray Kavukcuoglu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/OordVK17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {6306--6315},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Neural Discrete Representation Learning},
 url = {https://proceedings.neurips.cc/paper/2017/hash/7a98af17e63a0ac09ce2e96d03992fbc-Abstract.html},
 year = {2017}
}

@inproceedings{dunbar2019zero,
 author = {Ewan Dunbar and
Robin Algayres and
Julien Karadayi and
Mathieu Bernard and
Juan Benjumea and
Xuan{-}Nga Cao and
Lucie Miskic and
Charlotte Dugrain and
Lucas Ondel and
Alan W. Black and
Laurent Besacier and
Sakriani Sakti and
Emmanuel Dupoux},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/DunbarAKBBCMDOB19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-2904},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {1088--1092},
 publisher = {{ISCA}},
 timestamp = {Fri, 29 Jan 2021 00:00:00 +0100},
 title = {The Zero Resource Speech Challenge 2019: {TTS} Without {T}},
 url = {https://doi.org/10.21437/Interspeech.2019-2904},
 year = {2019}
}

@inproceedings{zhang2021uwspeech,
 author = {Zhang, Chen and Tan, Xu and Ren, Yi and Qin, Tao and Zhang, Kejun and Liu, Tie-Yan},
 booktitle = {Proc. of the AAAI},
 pages = {14319--14327},
 title = {Uwspeech: Speech to speech translation for unwritten languages},
 year = {2021}
}

@inproceedings{baevski2019vq,
 author = {Alexei Baevski and
Steffen Schneider and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/BaevskiSA20.bib},
 booktitle = {Proc. of ICLR},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {vq-wav2vec: Self-Supervised Learning of Discrete Speech Representations},
 url = {https://openreview.net/forum?id=rylwJxrYDS},
 year = {2020}
}

@article{meng2022cobert,
 author = {Meng, Chutong and Ao, Junyi and Ko, Tom and Wang, Mingxuan and Li, Haizhou},
 journal = {ArXiv preprint},
 title = {CoBERT: Self-Supervised Speech Representation Learning Through Code Representation Learning},
 url = {https://arxiv.org/abs/2210.04062},
 volume = {abs/2210.04062},
 year = {2022}
}

@article{lu2022unsupervised,
 author = {Lu, Zhiyun and Wang, Yongqiang and Zhang, Yu and Han, Wei and Chen, Zhehuai and Haghani, Parisa},
 journal = {ArXiv preprint},
 title = {Unsupervised Data Selection via Discrete Speech Representation for ASR},
 url = {https://arxiv.org/abs/2204.01981},
 volume = {abs/2204.01981},
 year = {2022}
}

@inproceedings{liu2019end,
 author = {Yuchen Liu and
Hao Xiong and
Jiajun Zhang and
Zhongjun He and
Hua Wu and
Haifeng Wang and
Chengqing Zong},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/LiuXZHWWZ19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-2582},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {1128--1132},
 publisher = {{ISCA}},
 timestamp = {Tue, 27 Jul 2021 01:00:00 +0200},
 title = {End-to-End Speech Translation with Knowledge Distillation},
 url = {https://doi.org/10.21437/Interspeech.2019-2582},
 year = {2019}
}

@inproceedings{ye2020variational,
 author = {Rong Ye and
Wenxian Shi and
Hao Zhou and
Zhongyu Wei and
Lei Li},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/YeS0W020.bib},
 booktitle = {Proc. of ICLR},
 publisher = {OpenReview.net},
 timestamp = {Wed, 09 Sep 2020 01:00:00 +0200},
 title = {Variational Template Machine for Data-to-Text Generation},
 url = {https://openreview.net/forum?id=HkejNgBtPB},
 year = {2020}
}

@article{hsu2021hubert,
 author = {Hsu, Wei-Ning and Bolte, Benjamin and Tsai, Yao-Hung Hubert and Lakhotia, Kushal and Salakhutdinov, Ruslan and Mohamed, Abdelrahman},
 journal = {IEEE/ACM Transactions on Audio, Speech, and Language Processing},
 pages = {3451--3460},
 publisher = {IEEE},
 title = {Hubert: Self-supervised speech representation learning by masked prediction of hidden units},
 volume = {29},
 year = {2021}
}

@inproceedings{vaswani2017attention,
 author = {Ashish Vaswani and
Noam Shazeer and
Niki Parmar and
Jakob Uszkoreit and
Llion Jones and
Aidan N. Gomez and
Lukasz Kaiser and
Illia Polosukhin},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/VaswaniSPUJGKP17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {5998--6008},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Attention is All you Need},
 url = {https://proceedings.neurips.cc/paper/2017/hash/3f5ee243547dee91fbd053c1c4a845aa-Abstract.html},
 year = {2017}
}

@article{liu2020multilingual,
 address = {Cambridge, MA},
 author = {Liu, Yinhan  and
Gu, Jiatao  and
Goyal, Naman  and
Li, Xian  and
Edunov, Sergey  and
Ghazvininejad, Marjan  and
Lewis, Mike  and
Zettlemoyer, Luke},
 doi = {10.1162/tacl_a_00343},
 journal = {Transactions of the Association for Computational Linguistics},
 pages = {726--742},
 publisher = {MIT Press},
 title = {Multilingual Denoising Pre-training for Neural Machine Translation},
 url = {https://aclanthology.org/2020.tacl-1.47},
 volume = {8},
 year = {2020}
}

@inproceedings{wang-etal-2020-fairseq,
 address = {Suzhou, China},
 author = {Wang, Changhan  and
Tang, Yun  and
Ma, Xutai  and
Wu, Anne  and
Okhonko, Dmytro  and
Pino, Juan},
 booktitle = {Proceedings of the 1st Conference of the Asia-Pacific Chapter of the Association for Computational Linguistics and the 10th International Joint Conference on Natural Language Processing: System Demonstrations},
 pages = {33--39},
 publisher = {Association for Computational Linguistics},
 title = {Fairseq {S}2{T}: Fast Speech-to-Text Modeling with Fairseq},
 url = {https://aclanthology.org/2020.aacl-demo.6},
 year = {2020}
}

@inproceedings{edunov-etal-2018-understanding,
 address = {Brussels, Belgium},
 author = {Edunov, Sergey  and
Ott, Myle  and
Auli, Michael  and
Grangier, David},
 booktitle = {Proc. of EMNLP},
 doi = {10.18653/v1/D18-1045},
 pages = {489--500},
 publisher = {Association for Computational Linguistics},
 title = {Understanding Back-Translation at Scale},
 url = {https://aclanthology.org/D18-1045},
 year = {2018}
}

@inproceedings{ao2022speecht5,
 address = {Dublin, Ireland},
 author = {Ao, Junyi  and
Wang, Rui  and
Zhou, Long  and
Wang, Chengyi  and
Ren, Shuo  and
Wu, Yu  and
Liu, Shujie  and
Ko, Tom  and
Li, Qing  and
Zhang, Yu  and
Wei, Zhihua  and
Qian, Yao  and
Li, Jinyu  and
Wei, Furu},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.393},
 pages = {5723--5738},
 publisher = {Association for Computational Linguistics},
 title = {{S}peech{T}5: Unified-Modal Encoder-Decoder Pre-Training for Spoken Language Processing},
 url = {https://aclanthology.org/2022.acl-long.393},
 year = {2022}
}

@inproceedings{caswell2019tagged,
 address = {Florence, Italy},
 author = {Caswell, Isaac  and
Chelba, Ciprian  and
Grangier, David},
 booktitle = {Proceedings of the Fourth Conference on Machine Translation (Volume 1: Research Papers)},
 doi = {10.18653/v1/W19-5206},
 pages = {53--63},
 publisher = {Association for Computational Linguistics},
 title = {Tagged Back-Translation},
 url = {https://aclanthology.org/W19-5206},
 year = {2019}
}

@inproceedings{kudo-richardson-2018-sentencepiece,
 address = {Brussels, Belgium},
 author = {Kudo, Taku  and
Richardson, John},
 booktitle = {Proc. of EMNLP},
 doi = {10.18653/v1/D18-2012},
 pages = {66--71},
 publisher = {Association for Computational Linguistics},
 title = {{S}entence{P}iece: A simple and language independent subword tokenizer and detokenizer for Neural Text Processing},
 url = {https://aclanthology.org/D18-2012},
 year = {2018}
}

@inproceedings{panayotov2015librispeech,
 author = {Vassil Panayotov and
Guoguo Chen and
Daniel Povey and
Sanjeev Khudanpur},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icassp/PanayotovCPK15.bib},
 booktitle = {2015 {IEEE} International Conference on Acoustics, Speech and Signal
Processing, {ICASSP} 2015, South Brisbane, Queensland, Australia,
April 19-24, 2015},
 doi = {10.1109/ICASSP.2015.7178964},
 pages = {5206--5210},
 publisher = {{IEEE}},
 timestamp = {Fri, 25 Dec 2020 00:00:00 +0100},
 title = {Librispeech: An {ASR} corpus based on public domain audio books},
 url = {https://doi.org/10.1109/ICASSP.2015.7178964},
 year = {2015}
}

@inproceedings{lee-etal-2022-textless,
 address = {Seattle, United States},
 author = {Lee, Ann  and
Gong, Hongyu  and
Duquenne, Paul-Ambroise  and
Schwenk, Holger  and
Chen, Peng-Jen  and
Wang, Changhan  and
Popuri, Sravya  and
Adi, Yossi  and
Pino, Juan  and
Gu, Jiatao  and
Hsu, Wei-Ning},
 booktitle = {Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
 doi = {10.18653/v1/2022.naacl-main.63},
 pages = {860--872},
 publisher = {Association for Computational Linguistics},
 title = {Textless Speech-to-Speech Translation on Real Data},
 url = {https://aclanthology.org/2022.naacl-main.63},
 year = {2022}
}

@inproceedings{zhang2022speechut,
 author = {Zhang, Ziqiang and Zhou, Long and Ao, Junyi and Liu, Shujie and Dai, Lirong and Li, Jinyu and Wei, Furu},
 booktitle = {Proc. of EMNLP},
 title = {Speechut: Bridging speech and text with hidden-unit for encoder-decoder based speech-text pre-training},
 year = {2022}
}

@inproceedings{post2018call,
 address = {Brussels, Belgium},
 author = {Post, Matt},
 booktitle = {Proceedings of the Third Conference on Machine Translation: Research Papers},
 doi = {10.18653/v1/W18-6319},
 pages = {186--191},
 publisher = {Association for Computational Linguistics},
 title = {A Call for Clarity in Reporting {BLEU} Scores},
 url = {https://aclanthology.org/W18-6319},
 year = {2018}
}

@misc{duh18multitarget,
 author = {Kevin Duh},
 howpublished = {\url{http://www.cs.jhu.edu/~kevinduh/a/multitarget-tedtalks/}},
 title = {The Multitarget TED Talks Task},
 year = {2018}
}

@inproceedings{sung2019towards,
 author = {Tzu{-}Wei Sung and
Jun{-}You Liu and
Hung{-}yi Lee and
Lin{-}Shan Lee},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icassp/SungLLL19.bib},
 booktitle = {{IEEE} International Conference on Acoustics, Speech and Signal Processing,
{ICASSP} 2019, Brighton, United Kingdom, May 12-17, 2019},
 doi = {10.1109/ICASSP.2019.8682801},
 pages = {7175--7179},
 publisher = {{IEEE}},
 timestamp = {Sun, 30 Jun 2019 01:00:00 +0200},
 title = {Towards End-to-end Speech-to-text Translation with Two-pass Decoding},
 url = {https://doi.org/10.1109/ICASSP.2019.8682801},
 year = {2019}
}

@inproceedings{salesky-etal-2019-exploring,
 address = {Florence, Italy},
 author = {Salesky, Elizabeth  and
Sperber, Matthias  and
Black, Alan W},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P19-1179},
 pages = {1835--1841},
 publisher = {Association for Computational Linguistics},
 title = {Exploring Phoneme-Level Speech Representations for End-to-End Speech Translation},
 url = {https://aclanthology.org/P19-1179},
 year = {2019}
}

@article{chen2020mam,
 author = {Chen, Junkun and Ma, Mingbo and Zheng, Renjie and Huang, Liang},
 journal = {ArXiv preprint},
 title = {Mam: Masked acoustic modeling for end-to-end speech-to-text translation},
 url = {https://arxiv.org/abs/2010.11445},
 volume = {abs/2010.11445},
 year = {2020}
}

@inproceedings{han-etal-2021-learning,
 address = {Online},
 author = {Han, Chi  and
Wang, Mingxuan  and
Ji, Heng  and
Li, Lei},
 booktitle = {Findings of ACL-IJCNLP 2021},
 doi = {10.18653/v1/2021.findings-acl.195},
 pages = {2214--2225},
 publisher = {Association for Computational Linguistics},
 title = {Learning Shared Semantic Space for Speech-to-Text Translation},
 url = {https://aclanthology.org/2021.findings-acl.195},
 year = {2021}
}

@inproceedings{sennrich-etal-2016-improving,
 address = {Berlin, Germany},
 author = {Sennrich, Rico  and
Haddow, Barry  and
Birch, Alexandra},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P16-1009},
 pages = {86--96},
 publisher = {Association for Computational Linguistics},
 title = {Improving Neural Machine Translation Models with Monolingual Data},
 url = {https://aclanthology.org/P16-1009},
 year = {2016}
}

@article{wu2022wav2seq,
 author = {Wu, Felix and Kim, Kwangyoun and Watanabe, Shinji and Han, Kyu and McDonald, Ryan and Weinberger, Kilian Q and Artzi, Yoav},
 journal = {ArXiv preprint},
 title = {Wav2Seq: Pre-training Speech-to-Text Encoder-Decoder Models Using Pseudo Languages},
 url = {https://arxiv.org/abs/2205.01086},
 volume = {abs/2205.01086},
 year = {2022}
}

@inproceedings{ren2020fastspeech,
 author = {Yi Ren and
Chenxu Hu and
Xu Tan and
Tao Qin and
Sheng Zhao and
Zhou Zhao and
Tie{-}Yan Liu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/0006H0QZZL21.bib},
 booktitle = {Proc. of ICLR},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {FastSpeech 2: Fast and High-Quality End-to-End Text to Speech},
 url = {https://openreview.net/forum?id=piLPYqxtWuA},
 year = {2021}
}

@inproceedings{kong2020hifi,
 author = {Jungil Kong and
Jaehyeon Kim and
Jaekyoung Bae},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/KongKB20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {HiFi-GAN: Generative Adversarial Networks for Efficient and High Fidelity
Speech Synthesis},
 url = {https://proceedings.neurips.cc/paper/2020/hash/c5d736809766d46260d816d8dbc9eb44-Abstract.html},
 year = {2020}
}

@inproceedings{chen2021gigaspeech,
 author = {Guoguo Chen and
Shuzhou Chai and
Guan{-}Bo Wang and
Jiayu Du and
Wei{-}Qiang Zhang and
Chao Weng and
Dan Su and
Daniel Povey and
Jan Trmal and
Junbo Zhang and
Mingjie Jin and
Sanjeev Khudanpur and
Shinji Watanabe and
Shuaijiang Zhao and
Wei Zou and
Xiangang Li and
Xuchen Yao and
Yongqing Wang and
Zhao You and
Zhiyong Yan},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/ChenCWDZWSPTZJK21.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-1965},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {3670--3674},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {GigaSpeech: An Evolving, Multi-Domain {ASR} Corpus with 10, 000 Hours
of Transcribed Audio},
 url = {https://doi.org/10.21437/Interspeech.2021-1965},
 year = {2021}
}

@article{kreuk2021textless,
 author = {Kreuk, Felix and Polyak, Adam and Copet, Jade and Kharitonov, Eugene and Nguyen, Tu-Anh and Rivi{\`e}re, Morgane and Hsu, Wei-Ning and Mohamed, Abdelrahman and Dupoux, Emmanuel and Adi, Yossi},
 journal = {ArXiv preprint},
 title = {Textless speech emotion conversion using decomposed and discrete representations},
 url = {https://arxiv.org/abs/2111.07402},
 volume = {abs/2111.07402},
 year = {2021}
}

@inproceedings{polyak2021speech,
 author = {Adam Polyak and
Yossi Adi and
Jade Copet and
Eugene Kharitonov and
Kushal Lakhotia and
Wei{-}Ning Hsu and
Abdelrahman Mohamed and
Emmanuel Dupoux},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/PolyakACKLHMD21.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-475},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {3615--3619},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {Speech Resynthesis from Discrete Disentangled Self-Supervised Representations},
 url = {https://doi.org/10.21437/Interspeech.2021-475},
 year = {2021}
}

@inproceedings{xia2019generalized,
 address = {Florence, Italy},
 author = {Xia, Mengzhou  and
Kong, Xiang  and
Anastasopoulos, Antonios  and
Neubig, Graham},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P19-1579},
 pages = {5786--5796},
 publisher = {Association for Computational Linguistics},
 title = {Generalized Data Augmentation for Low-Resource Translation},
 url = {https://aclanthology.org/P19-1579},
 year = {2019}
}

@article{tang2020multilingual,
 author = {Tang, Yuqing and Tran, Chau and Li, Xian and Chen, Peng-Jen and Goyal, Naman and Chaudhary, Vishrav and Gu, Jiatao and Fan, Angela},
 journal = {ArXiv preprint},
 title = {Multilingual translation with extensible multilingual pretraining and finetuning},
 url = {https://arxiv.org/abs/2008.00401},
 volume = {abs/2008.00401},
 year = {2020}
}

@inproceedings{chen2020facebook,
 address = {Online},
 author = {Chen, Peng-Jen  and
Lee, Ann  and
Wang, Changhan  and
Goyal, Naman  and
Fan, Angela  and
Williamson, Mary  and
Gu, Jiatao},
 booktitle = {Proceedings of the Fifth Conference on Machine Translation},
 pages = {113--125},
 publisher = {Association for Computational Linguistics},
 title = {{F}acebook {AI}{'}s {WMT}20 News Translation Task Submission},
 url = {https://aclanthology.org/2020.wmt-1.8},
 year = {2020}
}

@inproceedings{bojar2011improving,
 address = {Edinburgh, Scotland},
 author = {Bojar, Ond{\v{r}}ej  and
Tamchyna, Ale{\v{s}}},
 booktitle = {Proceedings of the Sixth Workshop on Statistical Machine Translation},
 pages = {330--336},
 publisher = {Association for Computational Linguistics},
 title = {Improving Translation Model by Monolingual Data},
 url = {https://aclanthology.org/W11-2138},
 year = {2011}
}

@inproceedings{bertoldi2009domain,
 address = {Athens, Greece},
 author = {Bertoldi, Nicola  and
Federico, Marcello},
 booktitle = {Proceedings of the Fourth Workshop on Statistical Machine Translation},
 pages = {182--189},
 publisher = {Association for Computational Linguistics},
 title = {Domain Adaptation for Statistical Machine Translation with Monolingual Resources},
 url = {https://aclanthology.org/W09-0432},
 year = {2009}
}

@inproceedings{sennrich2016improving,
 address = {Berlin, Germany},
 author = {Sennrich, Rico  and
Haddow, Barry  and
Birch, Alexandra},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P16-1009},
 pages = {86--96},
 publisher = {Association for Computational Linguistics},
 title = {Improving Neural Machine Translation Models with Monolingual Data},
 url = {https://aclanthology.org/P16-1009},
 year = {2016}
}

@inproceedings{hoang2018iterative,
 address = {Melbourne, Australia},
 author = {Hoang, Vu Cong Duy  and
Koehn, Philipp  and
Haffari, Gholamreza  and
Cohn, Trevor},
 booktitle = {Proceedings of the 2nd Workshop on Neural Machine Translation and Generation},
 doi = {10.18653/v1/W18-2703},
 pages = {18--24},
 publisher = {Association for Computational Linguistics},
 title = {Iterative Back-Translation for Neural Machine Translation},
 url = {https://aclanthology.org/W18-2703},
 year = {2018}
}

@inproceedings{imamura2018enhancement,
 address = {Melbourne, Australia},
 author = {Imamura, Kenji  and
Fujita, Atsushi  and
Sumita, Eiichiro},
 booktitle = {Proceedings of the 2nd Workshop on Neural Machine Translation and Generation},
 doi = {10.18653/v1/W18-2707},
 pages = {55--63},
 publisher = {Association for Computational Linguistics},
 title = {Enhancement of Encoder and Attention Using Target Monolingual Corpora in Neural Machine Translation},
 url = {https://aclanthology.org/W18-2707},
 year = {2018}
}

@inproceedings{adelani2022findings,
 author = {Adelani, David Ifeoluwa and Alam, Md Mahfuz Ibn and Anastasopoulos, Antonios and Bhagia, Akshita and Costa-Juss{\'a}, Marta and Dodge, Jesse and Faisal, Fahim and Federmann, Christian and Fedorova, Natalia and Guzm{\'a}n, Francisco and others},
 booktitle = {Proceedings of the Seventh Conference on Machine Translation, Online. Association for Computational Linguistics},
 title = {Findings of the WMT 2022 shared task on large-scale machine translation evaluation for african languages},
 year = {2022}
}

@inproceedings{wenzek2021findings,
 address = {Online},
 author = {Wenzek, Guillaume  and
Chaudhary, Vishrav  and
Fan, Angela  and
Gomez, Sahir  and
Goyal, Naman  and
Jain, Somya  and
Kiela, Douwe  and
Thrush, Tristan  and
Guzm{\'a}n, Francisco},
 booktitle = {Proceedings of the Sixth Conference on Machine Translation},
 pages = {89--99},
 publisher = {Association for Computational Linguistics},
 title = {Findings of the {WMT} 2021 Shared Task on Large-Scale Multilingual Machine Translation},
 url = {https://aclanthology.org/2021.wmt-1.2},
 year = {2021}
}

@inproceedings{farhad2021findings,
 address = {Copenhagen, Denmark},
 author = {Bojar, Ond{\v{r}}ej  and
Chatterjee, Rajen  and
Federmann, Christian  and
Graham, Yvette  and
Haddow, Barry  and
Huang, Shujian  and
Huck, Matthias  and
Koehn, Philipp  and
Liu, Qun  and
Logacheva, Varvara  and
Monz, Christof  and
Negri, Matteo  and
Post, Matt  and
Rubino, Raphael  and
Specia, Lucia  and
Turchi, Marco},
 booktitle = {Proceedings of the Second Conference on Machine Translation},
 doi = {10.18653/v1/W17-4717},
 pages = {169--214},
 publisher = {Association for Computational Linguistics},
 title = {Findings of the 2017 Conference on Machine Translation ({WMT}17)},
 url = {https://aclanthology.org/W17-4717},
 year = {2017}
}

@inproceedings{hayashi2018back,
 author = {Hayashi, Tomoki and Watanabe, Shinji and Zhang, Yu and Toda, Tomoki and Hori, Takaaki and Astudillo, Ramon and Takeda, Kazuya},
 booktitle = {2018 IEEE Spoken Language Technology Workshop (SLT)},
 organization = {IEEE},
 pages = {426--433},
 title = {Back-translation-style data augmentation for end-to-end ASR},
 year = {2018}
}

@inproceedings{ueno2021data,
 author = {Ueno, Sei and Mimura, Masato and Sakai, Shinsuke and Kawahara, Tatsuya},
 booktitle = {2021 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
 organization = {IEEE},
 pages = {68--75},
 title = {Data Augmentation for ASR Using TTS Via a Discrete Representation},
 year = {2021}
}

@inproceedings{tjandra2017listening,
 author = {Tjandra, Andros and Sakti, Sakriani and Nakamura, Satoshi},
 booktitle = {2017 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
 organization = {IEEE},
 pages = {301--308},
 title = {Listening while speaking: Speech chain by deep learning},
 year = {2017}
}

@inproceedings{zhang2022ustc,
 address = {Dublin, Ireland (in-person and online)},
 author = {Zhang, Weitai  and
Ye, Zhongyi  and
Tang, Haitao  and
Li, Xiaoxi  and
Zhou, Xinyuan  and
Yang, Jing  and
Cui, Jianwei  and
Deng, Pan  and
Shi, Mohan  and
Song, Yifan  and
Liu, Dan  and
Liu, Junhua  and
Dai, Lirong},
 booktitle = {Proceedings of the 19th International Conference on Spoken Language Translation (IWSLT 2022)},
 doi = {10.18653/v1/2022.iwslt-1.15},
 pages = {198--207},
 publisher = {Association for Computational Linguistics},
 title = {The {USTC}-{NELSLIP} Offline Speech Translation Systems for {IWSLT} 2022},
 url = {https://aclanthology.org/2022.iwslt-1.15},
 year = {2022}
}

@article{bapna2022mslam,
 author = {Bapna, Ankur and Cherry, Colin and Zhang, Yu and Jia, Ye and Johnson, Melvin and Cheng, Yong and Khanuja, Simran and Riesa, Jason and Conneau, Alexis},
 journal = {ArXiv preprint},
 title = {mSLAM: Massively multilingual joint pre-training for speech and text},
 url = {https://arxiv.org/abs/2202.01374},
 volume = {abs/2202.01374},
 year = {2022}
}

@article{babu2021xls,
 author = {Babu, Arun and Wang, Changhan and Tjandra, Andros and Lakhotia, Kushal and Xu, Qiantong and Goyal, Naman and Singh, Kritika and von Platen, Patrick and Saraf, Yatharth and Pino, Juan and others},
 journal = {ArXiv preprint},
 title = {XLS-R: Self-supervised cross-lingual speech representation learning at scale},
 url = {https://arxiv.org/abs/2111.09296},
 volume = {abs/2111.09296},
 year = {2021}
}

@inproceedings{li2021multilingual,
 address = {Online},
 author = {Li, Xian  and
Wang, Changhan  and
Tang, Yun  and
Tran, Chau  and
Tang, Yuqing  and
Pino, Juan  and
Baevski, Alexei  and
Conneau, Alexis  and
Auli, Michael},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.68},
 pages = {827--838},
 publisher = {Association for Computational Linguistics},
 title = {Multilingual Speech Translation from Efficient Finetuning of Pretrained Models},
 url = {https://aclanthology.org/2021.acl-long.68},
 year = {2021}
}

@inproceedings{ardila-etal-2020-common,
 address = {Marseille, France},
 author = {Ardila, Rosana  and
Branson, Megan  and
Davis, Kelly  and
Kohler, Michael  and
Meyer, Josh  and
Henretty, Michael  and
Morais, Reuben  and
Saunders, Lindsay  and
Tyers, Francis  and
Weber, Gregor},
 booktitle = {Proceedings of the Twelfth Language Resources and Evaluation Conference},
 isbn = {979-10-95546-34-4},
 language = {English},
 pages = {4218--4222},
 publisher = {European Language Resources Association},
 title = {Common Voice: A Massively-Multilingual Speech Corpus},
 url = {https://aclanthology.org/2020.lrec-1.520},
 year = {2020}
}

@inproceedings{ott2019fairseq,
 address = {Minneapolis, Minnesota},
 author = {Ott, Myle  and
Edunov, Sergey  and
Baevski, Alexei  and
Fan, Angela  and
Gross, Sam  and
Ng, Nathan  and
Grangier, David  and
Auli, Michael},
 booktitle = {Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics (Demonstrations)},
 doi = {10.18653/v1/N19-4009},
 pages = {48--53},
 publisher = {Association for Computational Linguistics},
 title = {fairseq: A Fast, Extensible Toolkit for Sequence Modeling},
 url = {https://aclanthology.org/N19-4009},
 year = {2019}
}

@inproceedings{bojar-EtAl:2016:WMT1,
 address = {Berlin, Germany},
 author = {Bojar, Ond{\v{r}}ej  and
Chatterjee, Rajen  and
Federmann, Christian  and
Graham, Yvette  and
Haddow, Barry  and
Huck, Matthias  and
Jimeno Yepes, Antonio  and
Koehn, Philipp  and
Logacheva, Varvara  and
Monz, Christof  and
Negri, Matteo  and
N{\'e}v{\'e}ol, Aur{\'e}lie  and
Neves, Mariana  and
Popel, Martin  and
Post, Matt  and
Rubino, Raphael  and
Scarton, Carolina  and
Specia, Lucia  and
Turchi, Marco  and
Verspoor, Karin  and
Zampieri, Marcos},
 booktitle = {Proceedings of the First Conference on Machine Translation: Volume 2, Shared Task Papers},
 doi = {10.18653/v1/W16-2301},
 pages = {131--198},
 publisher = {Association for Computational Linguistics},
 title = {Findings of the 2016 Conference on Machine Translation},
 url = {https://aclanthology.org/W16-2301},
 year = {2016}
}

@inproceedings{schwenk2019ccmatrix,
 address = {Online},
 author = {Schwenk, Holger  and
Wenzek, Guillaume  and
Edunov, Sergey  and
Grave, Edouard  and
Joulin, Armand  and
Fan, Angela},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.507},
 pages = {6490--6500},
 publisher = {Association for Computational Linguistics},
 title = {{CCM}atrix: Mining Billions of High-Quality Parallel Sentences on the Web},
 url = {https://aclanthology.org/2021.acl-long.507},
 year = {2021}
}

